Complete Log Concavity of Coverage-Like Functions

We introduce an expressive subclass of non-negative almost submodular set functions, called strongly 2-coverage functions which include coverage and (sums of) matroid rank functions, and prove that the homogenization of the generating polynomial of any such function is completely log-concave, taking a step towards characterizing the coefficients of (homogeneous) completely log-concave polynomials. As a consequence we obtain that the "level sets" of any such function form an ultra-log concave sequence.

==> technical-pre.tex <==

\section{Main Results}
\subsection{Strong Log-Concavity of  Homogeneous Parts}
Given  a non-negative  function  $f: 2^{[n]} \rightarrow \mathbb{R}$ and a set $\tau \subseteq [n]$,  define  \[S_{f, \tau}:=\{ e \in {[n]\setminus \tau}|  \exists S: f(  \tau \cup \{e\} \cup S) \neq  0\}.\]
Now, define $f_\tau: 2^{S_{f, \tau}} \rightarrow \mathbb{R}$  to be  $f_\tau (S) = f(S \cup \tau)$,  Furthermore, for any set function $f$,  define $f^d$ to be equal to $f$ on sets of size $d$ and $0$ otherwise. 
\begin{definition}[2-Coverage $d$-Homogeneous Measure ]
 A $d$-homogeneous measure $f^d$ is $2$-coverage if the following conditions hold.
 \begin{enumerate}[label=(\roman*)]
 \item
For all $\tau \subseteq [n]$ with $|\tau| \leq  d-2$, $(f^d)_\tau$ is indecomposable. 
\item
For all $\tau \subseteq [n]$ with $|\tau| = d-2$, there exists a coverage function $f'_\tau: 2^{[n] \setminus \tau} \rightarrow \mathbb{R} $,  such that  $(f^d)_\tau$ is the restriction of  $f'_\tau - c$, for  some constant $c$ such that $0 \leq c \leq \min f'_\tau(\{i\})$ for $i\in S_{f^d, \tau}$. 
\end{enumerate}
\end{definition}
\begin{theorem}\label{main}
Let $f : 2^{[n]} \rightarrow \mathbb{R}_{\geq 0}$. For  $2 \leq d $, $f^d$ is a strongly log-concave measure if it is $2$-coverage.
\end{theorem}
\begin{proof}
Let $p$ be the generating polynomial of $f^d$. We use  theorem \ref{log-concave-thm} to prove the theorem. 
Note that the indecomposability condition holds by definition. 
\par Now, we use lemma \ref{log-concave-lemma}  to prove that the second condition of   theorem \ref{log-concave-thm} holds.  Fix  $ \tau = i_1, \dots, i_{d-2}$. We want to show that $\partial^\tau p$ is log-concave.  If $\partial^\tau p$ is identically zero, the condition trivially holds. So, assume that $\partial^\tau p \neq 0$. Without loss of generality, we assume that  $\partial^\tau p$ is a $2$-homogeneous polynomial with  variables in $S_\tau$, and  $S_\tau = [m]$. We want to show that $\nabla^2 (\partial^\tau p)$ has at most one positive eigenvalue. We show this by writing  $\nabla^2 (\partial^\tau p)$ as  subtraction of some PSD matrices from a matrix with exactly  one positive eigenvalue.  
\par
Note that by assumption, for any $i,j \in [m]$,  $\nabla^2 (\partial^\tau p)( i, j) =   f'_\tau(\{i, j\}) - c$. Using lemma \ref{coverage-lemma}, there exists $x_T \geq 0$ for all $T \subseteq [m]$  such that
\begin{equation*}
f'_\tau(\{i, j\}) =\sum_{T: T \cap \{i,j\} \neq \emptyset} x_{T} =\sum_{T: T \cap \{i\} \neq \emptyset} x_{T} + \sum_{T: T \cap \{j\} \neq \emptyset} x_{T}  - \sum_{T: T \cap \{i,j\} = \{i,j\} } x_T 
\end{equation*}
\begin{equation} \label{dec}
= f'_\tau(\{i\}) +f'_\tau(\{j\})  -  \sum_{T: T \cap \{i,j\} = \{i,j\} } x_T 
\end{equation}
   Let $D$ be a diagonal matrix with $D(i,i) = f'_\tau(\{i\})$. Note that for all $i,j$,  $(DJ + JD) (i,j) =  f'_\tau(\{i\}) +f'_\tau(\{j\}) $. 
Therefore, we can write $\nabla^2(\partial^\tau p)$ as $(DJ + JD)  - R$, where on $R$ is defined as
\[R(i,i) =  2 f'_\tau(\{i\}),\]
on diagonal entries, and 
  \[R(i,j) = (\sum_{T: T \cap \{i,j\} = \{i,j\} } x_T )- c \]
   for $i \neq j$. First note that $DJ + JD$ has at most one positive eigenvalue. To see why, write 
\[JD+DJ = (D+I )J(D+I)  - DJD - J\]
Since $(D+I )J(D+I)$ is a rank $1$ matrix, it has at most one positive eigenvalue.  matrices $J$ and $DJD$ are rank $1$  and have positive entries, so they are PSD.  Now to prove $\nabla^2 (\partial^\tau p) $ has at most one positive eigenvalue, it is enough to show that $R$ is PSD. We show this by carefully writing $R$ as  summation of some PSD matrices. 
\par
Let  $D'$ be a diagonal matrix defined as $D'(i,i) =  f'_\tau(\{i\}) - c $. 
 Furthermore,  for any $T \subseteq [m]$ matrix $B_T$ is defined as  $B_T (i, j) = 1$ if $\{i,j\} \in T$ and $0$ otherwise. Using equation \ref{dec}, we can write $\nabla^2 (\partial^\tau p)$ as follows 
\[
R =  \sum_{T \subseteq[m]} x_T B_T  + cJ + D' 
\]
where $J \in \mathbb{R}^m$ is the all-one matrix. 
\par 
For any $T $, matrix $B_T$ is a rank $1$ PSD matrix.  Therefore,  since for all $T$, $x_T \geq 0$, matrix $\sum_{T \subseteq[m]} x_T B_T$ is PSD. Clearly, $cJ$ and $D'$ are also PSD matrices. Therefore, $R$ is PSD.
\end{proof}

\begin{theorem}
Let $f: 2^{[n]} \rightarrow \mathbb{R}$ be a non-negative monotone submodular function. Fix any $1 \leq d \leq n$. For any $0 \leq k \leq d$ and  $ \tau = i_1, \dots, i_k$, $(f^d)_\tau $  is  indecomposable. 
\end{theorem}
\begin{proof}
  Fix $2 \leq d \leq n$. For any $0 \leq k \leq d$ and $ \tau = i_1, \dots, i_k$, we want to show the polynomial  $\partial^\tau p := \partial_{i_1} \dots \partial_{i_k} p$ is indecomplosable.
If $\partial^\tau p$ is identically zero, it is also indecomposable. So, assume $\partial^\tau p \neq 0$.
Without loss of generality, we assume that  $\partial^\tau p$ is a $(d-k)$-homogeneous polynomial with  variables in $S_\tau$. The coefficient of any monomial $x^S$ in $\partial^\tau p$ is $f_\tau(S)$.   If  $f(\tau ) \neq 0$, all coefficients of $\partial^\tau p$ are non-zero and thus it is indecomposable. So, assume  $f(\tau) =0$. Since $\partial^\tau p \neq 0$, submodularity implies that there exists $j \in S_\tau$ such that $f(\{j\})>0$.  Let  $\partial^\tau p = g + h$ where $g$ and $h$ are non-zero.   Without loss of generality, $g$ has $x_j$. If $h$ also has $x_j$, $\partial^\tau p $ is indecomposable. So, assume that $h$ does not have $x_j$. Since $h$ is non-zero,  submodularity implies that $h$ has a variable $l$ such that $f(\{l \}) > 0$. Because of monotonicity, for any set $S$ such that $j, l\in S$, $f_\tau (S)$ is non-zero. Therefore $g$ has $x_l$ and  thus $\partial^\tau p $ is indecomposable. 
\end{proof}
\begin{corollary}\label{corollary1}
\begin{enumerate}[label=(\roman*)]
\item If $f: 2^{[n]} \rightarrow \mathbb{R}$ is a coverage function, for any $2 \leq d \leq n$, $f^d$ is a strongly log-concave measure. 
\item Let $M = ([n], I)$ be a matroid and  $ \operatorname{  rk}_M: 2^{[n]} \rightarrow \mathbb{R}$ be the rank function associated with $M$. For any $2 \leq d \leq \operatorname{rk}_M([n])$, $\operatorname{rk}_M^d$ is a strongly log-concave measure. 
\item We show that the strong log-concavity of bases generating polynomial of a matroid,  that is proven in \cite{10.1145/3313276.3316385}, is  a special case of this theorem. 
\end{enumerate}
\end{corollary}
\begin{proof}
\begin{enumerate}[label=(\roman*)]
\item 
We show that $f^d$ is a $2$-coverage measure. First, note that coverage functions are non-negative, monotone, and submodular. Therefore, the indecomposability condition holds. Now, we verify the second condition.   According to the definition of coverage functions, there exist $A_1, \dots, A_n \subseteq U$ and a measure $w$ such that for all $T \subseteq [n]$, $f(T) = w( \cup_{i \in T} A_i)$. For any $\tau \subseteq [n]$ with $|\tau| = d-2$, let $A_\tau = \cup_{i \in \tau} A_i$. Now, for any $i \in [n] \setminus \tau$, let $A^\prime_i = A_i \cup A_\tau$, and for any $S \subseteq [n] \setminus \tau$, let $f'_\tau(S) = w(\cup_{i \in S} A_i^\prime)$. 
\item Let $f:= \operatorname{  rk}_M$. For any $\tau \subseteq [n]$ with $|\tau| = d-2$, $(f^d)_\tau (S) = \operatorname{rk}_M(\tau) + \operatorname{rk}_{M/\tau}(S)$ for all size-$2$ set $S \subseteq [n] \setminus \tau$. Using matroid partition property, $M/\tau$ can be partitioned into sets $S_0, \dots, S_k$ such that the following holds. 
\[
\operatorname{rk}_{M/\tau}(\{x, y\}) = 
     \begin{cases}
       \text{0} &\quad x, y \in S_0\\
       \text{1} &\quad  x\in S_0, y\in S_i \quad \text{for some } 1\leq i\leq k \\
       \text{1} &\quad x, y \in S_i \quad \text{for some } 1\leq i\leq k\\
       \text{2} &\quad x \in S_i, y \in S_j \quad \text{for some} 1\leq i< j \leq k\\ 
     \end{cases}
\]
Now we extend $f_\tau^2 (.)$ to a coverage function as follows. Take the universe to be $[k+1] \cup \{-1\}$ and define the measure $w_\tau$ to be $w_\tau (\{-1\}) = \operatorname{rk}_M(\tau)$, $w_\tau(\{0\}) = 0$, and   $w_\tau(\{i\}) = 1$ for all $1\leq i\leq k$. Now, for any $ i \in [k+1]$ and $x \in S_i$, let $A_x := \{-1, i\}$. For any $S \in [n] \setminus \tau$ the coverage function is defined as  $f'_\tau(S)  = w_\tau(\cup_{i \in S} A_i)$. 
\item
 Let $M = ([n], I)$ be a matroid of rank $r$ and let
$f: 2^{[n]} \rightarrow \mathbb{R}$ be an indicator function of independent sets, i.e. $f(S) = \mathbf{1}_I$. We want to show that $f^r$ is a $2$-coverage measure. The indecomposability holds because of the exchange property of matroids. We verify the second condition. Note that for any $\tau \subseteq [n]$ with $|\tau| = d-2$, using the matroid partition property,  non-loop elements of $M/\tau$ which correspond to $S_{f, \tau}$  can be partitioned into sets $S_1, \dots, S_k$  such that 
\[
(f^d)_{\tau}(\{x, y\}) = 
     \begin{cases}
    
       \text{0} &\quad x, y \in S_i \quad \text{for some } 1\leq i\leq k\\
       \text{1} &\quad x \in S_i, y \in S_j \quad \text{for some } 1\leq i< j \leq k\\ 
     \end{cases}
\]
Now we extend $(f^d)_{\tau} (.)$ to a coverage function as follows. Take the universe to be $\{1, \dots, k\}$ and define the measure $w_\tau$ to be  $w_\tau(\{i\}) = 1$ for all $i$ in the universe. Now, for any $ 1 \leq i \leq k$ and $x \in S_i$, let $A_x := \{ i\}$. For any $S \in [n] \setminus \tau$ the coverage function is defined as  $f'_\tau(S)  = w_\tau(\cup_{i \in S} A_i)$. 
\end{enumerate}
\end{proof}


\section{Negative results}

There is a counter-example to the  natural generalization of our result for any positive monotone submodular measure, as follows. 
any  positive monotone submodular measure. 
\begin{lemma}
There exists a non-negative monotone submodular function $f$ such that its restriction to sets of size $d$, i.e. $f^d$, is not a log-concave measure. 
\end{lemma}
\begin{proof}
Let $[12]$ be the ground set. Furthermore, define $w_0 = \dots = w_5 = 1$, $w_6 = \dots = w_9 = 2$, and $w_{10} = w_{11} = 0$. Now, take the following set function $f: 2^{[12] }\rightarrow \mathbb{R}$ to be $f(S) =\max \{ \sum_{i \in s}  w_i, 2\}$. Note that this function is a budget additive function and is non-negative, monotone  and submodular. But, one can verify that the polynomial $p(x) = \sum_{\{i,j\} \subseteq [12] } f(\{i,j\})$ is not log-concave. 

\end{proof}
Gelfand, Goresky, MacPherson, and Serganova proved that the support of any homogeneous multilinear log-concave polynomial correspond to bases of a matroid \cite{GELFAND1987301}. But there is not much known about the coefficient of these polynomials. A natural question to ask is that if the coefficients come from a   monotone submodular function that is non-negative on non-empty sets. The following lemma provides a counter-example to this statement. 
\begin{lemma}
There exists a $2$-homogeneous multilinear log-concave $p \in R_{\geq 0}[x_1, x_2, x_3]$, such that if we define function $f_p$ on any  $S\subseteq \{1, 2, 3\}$ of size $2$ to be coefficient of the monomial $x^S$, then $f$ cannot be extended to a monotone submodular function that is non-negative on non-empty sets.
\end{lemma}
\begin{proof}
Let $p (x1, x_2, x_3) := 3 x_1x_2 +   x_2x_3 + x_2x_3$. We have 
\[
\nabla^2 p = \begin{bmatrix}
0 & 3 & 1\\
3 & 0 & 1\\
1 & 1 & 0\\
\end{bmatrix},
\]
which has exactly 1 positive eigenvalue, so using \label{log-concave-lemma} $p$ is log-concave. Now, let $f'_p$ be an extension of $f_p$ that is  monotone and   non-negative on non-empty sets. We have $f(\{1, 2, 3\}) -  f(\{1, 3\})  \geq 2$. On the other hand,  $f(\{2, 3\})  -f(\{3\})  \leq 1$. So,   $f$ is not submodular. 

\end{proof}
\section{Entropy as a Coverage Function}
Given random variables $\Omega = \{ Y_1, \dots, Y_n\}$, let $H: 2^{\Omega } \rightarrow \mathbb{R}_{\geq 0}$ be the entropy function. 
\begin{lemma}
Let  $f: 2^{[n]} \rightarrow \mathbb{R}_{\geq 0}$ defined as $f(S) = H(Y_S)$ for any $S\subseteq [n]$, where $Y_S:= \{Y_i| i \in S\}$. Then, $f$ is a coverage function. 
 \end{lemma}
\begin{proof}
We use the equivalent condition in  lemma \ref{coverage-lemma}.
Recall that multivariate mutual information is defined inductively as
\[I(X|Y) := H(X|Y)\]
\[
I(X_1, \dots, X_n|Y) :=  I(X_1, \dots, X_{n-1}|Y) - I(X_1, \dots, X_{n-1}| X_n, Y).
\]
 For any $T \subseteq [n]$, we define $x_T := I(Y_T|Y_{\bar{T}})$. We argue that for any $S \subseteq [n]$, $f(S) = \sum_{T: T\cap S \neq \emptyset} x_T$. We prove inductively that $H(Y_S |Z ) = \sum_{T: T\cap S \neq \emptyset} I(Y_S| Y_{\bar{S}}, Z)$. When $n =1$, it trivially holds. We assume it is true for $n = k-1$ and prove it for for $n=k$. First, let $S=\{i\}$. We have
 \[
\sum_{T: T\cap S \neq \emptyset} I(Y_T \mid Y_{\bar{T}})= \sum_{T: i \in T} I(Y_T \mid Y_{\bar{T}}) = (\sum_{T: i \in T, T \neq \{i\}} I(Y_{T \setminus \{i\}} | Y_{\bar{T}})  -  I(Y_{T \setminus \{i\}} | Y_{\bar{T} \cup \{i\}}) )+ H(Y_i | Y_{\bar{i}}).
\]
Using induction hypothesis
\[\sum_{T: i \in T, T \neq \{i\}} I(Y_{T \setminus \{i\}} | Y_{\bar{T}})  -  I(Y_{T \setminus \{i\}} | Y_{\bar{T} \cup \{i\}})=  H(Y_{[n] \setminus \{i \}}) -  H(Y_{[n] \setminus\{ i\} }| Y_{ \{i\}}) \]
\[
 = H(Y_{[n] \setminus \{i\}}) - H(Y_{[n]}) + H(Y_i)  =  H(Y_{[n]} \mid Y_{[n] \setminus \{i\}}) .
\]
Therefore, 
\[
\sum_{T: T\cap S \neq \emptyset} I(Y_T \mid Y_{\bar{T}}) = H(Y_i).
\]
Now, assume that this equation holds for any  $S$ such that $|S| <l$. We want to show that it holds for $|S| = l$.  Choose $i \in S$.  We have
\[
\sum_{T: T\cap S \neq \emptyset} I(Y_T \mid Y_{\bar{T}}) =\sum_{T: T\cap ( S \setminus \{i\}) \neq \emptyset} I(Y_T | Y_{\bar{T}}) + \sum_{T \cap S = \{i\}}  I(Y_T | Y_{\bar{T}}).
\]
Note that $\sum_{T: T\cap ( S \setminus \{i\}) \neq \emptyset} I(Y_T | Y_{\bar{T}}) = H(Y_{S \setminus \{i\}}) $ by  the second induction hypothesis. Furthermore,
\[
 \sum_{T \cap S = \{i\}}  I(Y_T | Y_{\bar{T}}) =  (\sum_{T \cap S = \{i\}, T \neq \{i\}}   I(Y_{T \setminus \{i\}} | Y_{\bar{T}})  -  I(Y_{T \setminus \{i\}} | Y_{\bar{T} \cup \{i\}}) )+ H(Y_i | Y_{\bar{i}}).
\]
Similar to what we did before, using the first induction hypothesis we get
\[
\sum_{T \cap S = \{i\}, T \neq \{i\}}   I(Y_{T \setminus \{i\}} | Y_{\bar{T}})  -  I(Y_{T \setminus \{i\}} | Y_{\bar{T} \cup \{i\}}) = 
H(Y_{[n] \setminus S } \mid Y_{S \setminus \{i\}}) -  H(Y_{[n] \setminus S }| Y_{S}) 
\]
\[ =  H(Y_{[n] \setminus S } \mid Y_{S \setminus \{i\}}) -  H(Y_{([n] \setminus S) \cup \{i\}} \mid Y_{S \setminus \{i\}}) + H( Y_{ i} \mid Y_{S \setminus \{i\}})) 
\]
\[
=-H\left(Y_{i} \mid Y_{[n] \backslash \{i\}}\right)+H( Y_{ i} \mid Y_{S \setminus \{i\}})).
\]
Therefore, 
\[
\sum_{T \cap S = \{i\}}  I(Y_T | Y_{\bar{T}})  = H( Y_{ i} \mid Y_{S \setminus \{i\}})).
\]
So 
\[
\sum_{T: T\cap S \neq \emptyset} I(Y_T \mid Y_{\bar{T}}) =H( Y_{ i} \mid Y_{S \setminus \{i\}})) +  H(Y_{S \setminus \{i\}})  = H(S) 
\]
\end{proof}
\subsection{Strong Log-Concavity of the Homogenized Measure}

\begin{definition}[ Strongly $2$- Coverage Measure]
 A  measure $f: 2^{[n]} \rightarrow \mathbb{R \geq 0 }$ is strongly $2$-coverage if the following holds.
 \par
For all $\tau \subseteq [n]$ such that $0 \leq |\tau| \leq n-2$,  there exists a coverage function $f'_\tau: 2^{[n] \setminus \tau} \rightarrow \mathbb{R} $,  such that   $(f^{|\tau|+1} )_\tau$ is the restriction of $f'_\tau + f(\tau) $, and  $(f^{|\tau|+2} )_\tau$ is the restriction of  $f'_\tau  + f(\tau)$. 
\end{definition}
\begin{lemma}
Coverage functions are strongly $2$-coverage. Furthermore, for any matroid $M=([n], I)$, $\operatorname{rk_M}$ is  strongly $2$-coverage.
\end{lemma}
\begin{proof}
The proof is similar to \ref{corollary1} [ToDo]. 
\end{proof}

\begin{theorem}
Let $f: 2^{[n]} \rightarrow \mathbb{R_{\geq 0}}$ be  a strongly $2$-coverage measure. Then, the polynomial $ p_f (y, x_1, \dots, x_n) = \sum_{i=0}^n y^ {n+2 -i} \sum_{S \subseteq [n], |S| = i} f(S) x^S$ is strongly log-concave. 

\end{theorem}
\begin{proof}
We use theorem \ref{log-concave-theorem}. First note that the indecomposability condition  follows from the definition [ToDo]. We prove that the second condition holds. It is enough to show that  for any  $0 \leq l \leq n$ and  $\tau = \{i_1 \dots, i_l\}$, $ \partial^\tau \partial ^{n - l} p_f (y, x)$ is log-concave. $q = \frac{\partial^\tau \partial ^{n - l} p_f (y, x)}{(n+1)!}$. We see that 
\[
q  = \frac{(n+2)n(n+1)}{2} f(\tau)  y^{2}+(n +1) \sum_{i  \in S_{f, \tau}} f (\tau \cup \{i\}) y x_{i}+ \sum_{  \{i, j\}  \subseteq S_{f, \tau}} f (\tau \cup \{i, j\}) x_{i} x_{j}.
\]
Without loss of generality assume that $S_{f, \tau} = \{1, \dots, m\}$, and note that $m \leq n-l$.  We compute the Hessian matrix 
\[ H = 
\begin{bmatrix}
(n+2)(n+1) f(\tau) & (n+1)) f_\tau(  \{1\})  & \dots & (n+1) f_\tau(  \{m\})\\
(n+1) f_\tau(  \{1\}) & 0 & \dots  &  f_\tau(  \{1, m \}) \\
\vdots &\vdots & \dots & \vdots  \\
(n+1) f_\tau(  \{m\}) & f_\tau(   \{m, 1 \})  & \dots  &  0\\
\end{bmatrix}
\]
Let $D =\operatorname{diag}(\begin{bmatrix} \frac{1}{n+1} & 1 &  \dots & 1 \end{bmatrix}^T)$. Note that it is enough to show that $H' = D HD$ has at most one positive eigenvalue [ToDo]. . By definition, there is coverage function $f'_\tau$ such that
\[ H' = 
\begin{bmatrix}
\frac{n+2}{n+1} f(\tau) & f'_\tau(  \{1\})+f(\tau)  & \dots &  f'_\tau(  \{m\}) + f(\tau)\\
 f'_\tau(  \{1\})+ f(\tau) & 0 & \dots  &  f'_\tau(  \{1, m \})+f(\tau)  \\
\vdots &\vdots & \dots & \vdots  \\
 f'_\tau(  \{m\}) +f(\tau) & f'_\tau(   \{m, 1 \})+f(\tau)   & \dots  &  0
\end{bmatrix} \]
\[ = \begin{bmatrix}
0 & f'_\tau(  \{1\}) & \dots &  f'_\tau(  \{m\}) \\
 f'_\tau(  \{1\}) & 0 & \dots  &  f'_\tau(  \{1, m \}) \\
\vdots &\vdots & \dots & \vdots  \\
 f'_\tau(  \{m\}) & f'_\tau(   \{m, 1 \})  & \dots  &  0\\
\end{bmatrix} 
+ \begin{bmatrix}
\frac{n+2}{n+1} f(\tau) & f(\tau)  & \dots &  f(\tau)\\
 f(\tau) & 0 & \dots  &f(\tau)  \\
\vdots &\vdots & \dots & \vdots  \\
 f(\tau) & f(\tau)   & \dots  &  0
\end{bmatrix} = H'_1 + H'_2
\]
Let $D' \in R^{(n+1) \times (n+1)}$ be a diagonal matrix with $D'(1,1) = f(\tau)$ and $D'(i,i) = f(\tau) + f'_\tau(\{i\})$. Note that $D'J + JD'$ has exactly one positive eigenvalue and
\[
D'J + JD' = f(\tau) J + \begin{bmatrix}
0 & f'_\tau(  \{1\}) & \dots &  f'_\tau(  \{m\}) \\
 f'_\tau(  \{1\}) & 2f'_\tau(  \{1\}) & \dots  &  f'_\tau(  \{1\})+f'_\tau(  \{m\}) \\
\vdots &\vdots & \dots & \vdots  \\
 f'_\tau(  \{m\}) &f'_\tau(  \{1\})+f'_\tau(  \{m\}) & \dots  &  2f'_\tau(  \{m\}) \\
\end{bmatrix}  = f(\tau) J + C.
\]
We show that we can write $H' =  f(\tau) J + C - (R_1 + R_2)$ for two PSD matrices $R_1$ and $R_2$. More specifically, we show that $H'_1 = C  - R_1$ and $H'_2 = f(\tau) J - R_2$, for two PSD matrices $R_1$ and $R_2$. First, note that $H'_1$ is the Hessian matrix of $p_{g^2}$ for a coverage function $g$ [ToDo]. Now, if we follow the steps of proof of \ref{main} for $g^2$, one can check that $R_1$ here is exactly  same as matrix $R$ in the proof of \ref{main}. So, $R_1$ is PSD. To check that $R_2$ is PSD, it is enough to show that for any $k$, the $k \times k$ matrix $A = J+ \operatorname{diag}(\begin{bmatrix} \frac{k-1}{k} & 2 & \dots &2  \end{bmatrix}^T)$ is PSD. This can be check by solving $A x= \lambda x$ [ToDo]. 

\begin{theorem}
Let $f: 2^{[n]} \rightarrow \mathbb{R_{\geq 0}}$ be  a strongly $2$-coverage measure. Let $c_k$ be the $k$-th coefficient of  $ p_f (y, x) = \sum_{i=0}^n y^ {n+2 -i} \sum_{S \subseteq [n], |S| = i} f(S) x^i$ is strongly log-concave. Then, for $1<k<n$, we get
\[
\left( \frac{c_k}{{n +2\choose k} }\right)^2 \geq  \left(\frac{c_{k-1}}{{n +2\choose k-1} }\right)\left(\frac{c_{k+1}}{{n +2\choose k+1} }\right)
\]

\end{theorem}
\end{proof}

